GNNDelete: A General Strategy for Unlearning in Graph Neural Networks

Graph unlearning, which involves deleting graph elements such as nodes, node labels, and relationships from a trained graph neural network (GNN) model, is crucial for real-world applications where data elements may become irrelevant, inaccurate, or privacy-sensitive. However, existing methods for graph unlearning either deteriorate model weights shared across all nodes or fail to effectively delete edges due to their strong dependence on local graph neighborhoods. To address these limitations, we introduce GNNDelete, a novel model-agnostic layer-wise operator that optimizes two critical properties, namely, Deleted Edge Consistency and Neighborhood Influence, for graph unlearning. Deleted Edge Consistency ensures that the influence of deleted elements is removed from both model weights and neighboring representations, while Neighborhood Influence guarantees that the remaining model knowledge is preserved after deletion. GNNDelete updates representations to delete nodes and edges from the model while retaining the rest of the learned knowledge. We conduct experiments on seven real-world graphs, showing that GNNDelete outperforms existing approaches by up to 38.8% (AUC) on edge, node, and node feature deletion tasks, and 32.2% on distinguishing deleted edges from non-deleted ones. Additionally, GNNDelete is efficient, taking 12.3x less time and 9.3x less space than retraining GNN from scratch on WordNet18.

==> cs.tex <==
% \begin{table}[h]
%   \caption{\textbf{Unlearning task: edge deletion when $\mathcal{E}_d = \mathcal{E}_{d, \texttt{OUT}}$. Evaluation: link prediction. Dataset: CS}. Reported is AUROC ($\uparrow$) performance with the best marked in \textbf{bold} and the second best \underline{underlined}.} 
%   \label{tab:full_result_cs}
%   \centering
%   \footnotesize
%   \setlength{\tabcolsep}{3.9pt}
%   \renewcommand{\arraystretch}{0.9}
%   \begin{tabular}{llcccccc}
%     \toprule
%     \multirow{2}{*}{Model} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{GAT} & \multicolumn{2}{c}{GIN} \\
%      & $\mathcal{E}_t$ & $\mathcal{E}_d$ & $\mathcal{E}_t$ & $\mathcal{E}_d$ & $\mathcal{E}_t$ & $\mathcal{E}_d$ \\
%     \midrule
%     \rowcolor{Gray}
%     \cellcolor{white}\multirow{6}{*}{0.5}
%     & \tabRetrain        & 0.967 \std{0.001} & 0.740 \std{0.017} & 0.960 \std{0.002} & 0.654 \std{0.017} & 0.962 \std{0.001} & 0.807 \std{0.014} \\
%     & \tabGradientAscent & 0.590 \std{0.012} & 0.667 \std{0.019} & 0.512 \std{0.015} & 0.553 \std{0.043} & 0.749 \std{0.011} & 0.814 \std{0.043} \\
%     & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
%     & \tabGraphEraser    & 0.532 \std{0.002} & 0.500 \std{0.000} & 0.527 \std{0.013} & 0.500 \std{0.000} & 0.515 \std{0.009} & 0.500 \std{0.000} \\
%     & \tabGraphEditor    & 0.614 \std{0.117} & 0.520 \std{0.031} & 0.614 \std{0.117} & 0.520 \std{0.031} & 0.614 \std{0.117} & 0.520 \std{0.031} \\
%     & \tabOurs           & 0.958 \std{0.001} & 0.967 \std{0.003} & 0.954 \std{0.001} & 0.965 \std{0.002} & 0.954 \std{0.002} & 0.960 \std{0.002} \\
    
%     \midrule
%     \rowcolor{Gray}
%     \cellcolor{white}\multirow{6}{*}{2.5} 
%     & \tabRetrain        & 0.967 \std{0.001} & 0.766 \std{0.008} & 0.960 \std{0.001} & 0.671 \std{0.006} & 0.961 \std{0.002} & 0.840 \std{0.006} \\
%     & \tabGradientAscent & 0.644 \std{0.087} & 0.652 \std{0.056} & 0.507 \std{0.011} & 0.505 \std{0.010} & 0.678 \std{0.013} & 0.587 \std{0.039} \\
%     & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
%     & \tabGraphEraser    & 0.542 \std{0.002} & 0.500 \std{0.000} & 0.519 \std{0.013} & 0.500 \std{0.000} & 0.563 \std{0.009} & 0.500 \std{0.000} \\
%     & \tabGraphEditor    & 0.614 \std{0.117} & 0.517 \std{0.025} & 0.614 \std{0.117} & 0.517 \std{0.025} & 0.614 \std{0.117} & 0.517 \std{0.025} \\
%     & \tabOurs           & 0.953 \std{0.002} & 0.893 \std{0.003} & 0.949 \std{0.001} & 0.871 \std{0.008} & 0.951 \std{0.003} & 0.921 \std{0.003} \\
    
%     \midrule
%     \rowcolor{Gray}
%     \cellcolor{white}\multirow{6}{*}{5.0}
%     & \tabRetrain        & 0.967 \std{0.001} & 0.787 \std{0.006} & 0.960 \std{0.002} & 0.688 \std{0.006} & 0.962 \std{0.001} & 0.864 \std{0.005} \\
%     & \tabGradientAscent & 0.665 \std{0.097} & 0.630 \std{0.067} & 0.533 \std{0.097} & 0.517 \std{0.064} & 0.667 \std{0.008} & 0.555 \std{0.036} \\
%     & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
%     & \tabGraphEraser    & 0.514 \std{0.002} & 0.500 \std{0.000} & 0.523 \std{0.013} & 0.500 \std{0.000} & 0.533 \std{0.009} & 0.500 \std{0.000} \\
%     & \tabGraphEditor    & 0.614 \std{0.117} & 0.515 \std{0.026} & 0.614 \std{0.117} & 0.515 \std{0.026} & 0.614 \std{0.117} & 0.515 \std{0.026}  \\
%     & \tabOurs           & 0.958 \std{0.004} & 0.862 \std{0.004} & 0.951 \std{0.002} & 0.821 \std{0.008} & 0.950 \std{0.001} & 0.916 \std{0.002} \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}[h]
  \caption{\textbf{Unlearning task: edge deletion when $\mathcal{E}_d = \mathcal{E}_{d, \texttt{OUT}}$. Evaluation: link prediction. Dataset: CS}. Reported is AUROC ($\uparrow$) performance with the best marked in \textbf{bold} and the second best \underline{underlined}.} 
  \label{tab:full_result_cs2}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{3.9pt}
  \renewcommand{\arraystretch}{0.9}
  \begin{tabular}{llcccccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{GCN} & \multicolumn{2}{c}{GAT} & \multicolumn{2}{c}{GIN} \\
     & $\mathcal{E}_t$ & $\mathcal{E}_d$ & $\mathcal{E}_t$ & $\mathcal{E}_d$ & $\mathcal{E}_t$ & $\mathcal{E}_d$ \\
    \midrule
    \rowcolor{Gray}
    \cellcolor{white}\multirow{6}{*}{0.5}
    & \tabRetrain        & 0.965 \std{0.002} & 0.511 \std{0.024} & 0.961 \std{0.001} & 0.513 \std{0.024} & 0.960 \std{0.003} & 0.571 \std{0.028} \\
    & \tabGradientAscent & 0.528 \std{0.008} & 0.588 \std{0.014} & 0.502 \std{0.002} & 0.543 \std{0.058} & 0.792 \std{0.046} & 0.705 \std{0.113} \\
    & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
    & \tabGraphEraser    & 0.528 \std{0.002} & 0.500 \std{0.000} & 0.523 \std{0.013} & 0.500 \std{0.000} & 0.542 \std{0.009} & 0.500 \std{0.000} \\
    & \tabGraphEditor    & 0.673 \std{0.191} & 0.488 \std{0.027} & 0.673 \std{0.191} & 0.488 \std{0.027} & 0.673 \std{0.191} & 0.488 \std{0.027} \\
    & \tabOurs           & 0.944 \std{0.003} & 0.843 \std{0.015} & 0.937 \std{0.004} & 0.880 \std{0.011} & 0.942 \std{0.005} & 0.824 \std{0.021} \\
    
    \midrule
    \rowcolor{Gray}
    \cellcolor{white}\multirow{6}{*}{2.5} 
    & \tabRetrain        & 0.966 \std{0.002} & 0.520 \std{0.008} & 0.961 \std{0.001} & 0.520 \std{0.012} & 0.958 \std{0.002} & 0.583 \std{0.007} \\
    & \tabGradientAscent & 0.509 \std{0.006} & 0.509 \std{0.007} & 0.490 \std{0.007} & 0.551 \std{0.014} & 0.639 \std{0.077} & 0.614 \std{0.016} \\
    & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
    & \tabGraphEraser    & 0.517 \std{0.002} & 0.500 \std{0.000} & 0.556 \std{0.013} & 0.500 \std{0.000} & 0.547 \std{0.009} & 0.500 \std{0.000} \\
    & \tabGraphEditor    & 0.673 \std{0.191} & 0.493 \std{0.027} & 0.673 \std{0.191} & 0.493 \std{0.027} & 0.673 \std{0.191} & 0.493 \std{0.027} \\
    & \tabOurs           & 0.925 \std{0.006} & 0.716 \std{0.003} & 0.928 \std{0.007} & 0.738 \std{0.005} & 0.919 \std{0.004} & 0.745 \std{0.005} \\
    
    \midrule
    \rowcolor{Gray}
    \cellcolor{white}\multirow{6}{*}{5.0}
    & \tabRetrain        & 0.964 \std{0.002} & 0.525 \std{0.008} & 0.960 \std{0.001} & 0.525 \std{0.007} & 0.958 \std{0.002} & 0.591 \std{0.006} \\
    & \tabGradientAscent & 0.509 \std{0.005} & 0.487 \std{0.003} & 0.489 \std{0.015} & 0.537 \std{0.007} & 0.592 \std{0.031} & 0.583 \std{0.013} \\
    & \tabDtD            & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} & 0.500 \std{0.000} \\
    & \tabGraphEraser    & 0.528 \std{0.002} & 0.500 \std{0.000} & 0.517 \std{0.013} & 0.500 \std{0.000} & 0.530 \std{0.009} & 0.500 \std{0.000} \\
    & \tabGraphEditor    & 0.673 \std{0.191} & 0.489 \std{0.023} & 0.673 \std{0.191} & 0.489 \std{0.023} & 0.673 \std{0.191} & 0.489 \std{0.023} \\
    & \tabOurs           & 0.916 \std{0.007} & 0.680 \std{0.006} & 0.920 \std{0.005} & 0.700 \std{0.004} & 0.900 \std{0.005} & 0.717 \std{0.003} \\
    \bottomrule
  \end{tabular}
\end{table}
